Quality Analysis of the Coding Bitrate Tradeoff Between Geometry and Attributes for Colored Point Clouds

Typically, point cloud encoders allocate a similar bitrate for geometry and attributes (usually RGB color components) information coding. This paper reports a quality study considering different coding bitrate tradeoff between geometry and attributes. A set of five point clouds, representing different characteristics and types of content was encoded with the MPEG standard Geometry Point Cloud Compression (G-PCC), using octree to encode geometry information, and both the Region Adaptive Hierarchical Transform and the Prediction Lifting transform for attributes. Furthermore, the JPEG Pleno Point Cloud Verification Model was also tested. Five different attributes/geometry bitrate tradeoffs were considered, notably 70%/30%, 60%/40%, 50%/50%, 40%/60%, 30%/70%. Three point cloud objective metrics were selected to assess the quality of the reconstructed point clouds, notably the PSNR YUV, the Point Cloud Quality Metric, and GraphSIM. Furthermore, for each encoder, the Bjonteegaard Deltas were computed for each tradeoff, using the 50%/50% tradeoff as a reference. The reported results indicate that using a higher bitrate allocation for attribute encoding usually yields slightly better results.

==> backupTabelas.tex <==
\begin{table*}[!t]
    \centering
    \Huge
    \caption{Parameters for G-PCC lifting transform.}
   \resizebox{\linewidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Parameter & \multicolumn{4}{|c|}{\textbf{Bouquet}}& \multicolumn{4}{|c|}{\textbf{StMihcael}}& \multicolumn{4}{|c|}{\textbf{Thaidancer}}& \multicolumn{4}{|c|}{\textbf{CITIUSP}} & \multicolumn{4}{|c|}{\textbf{Bumbameuboi}}\\ \hline
    &\multicolumn{20}{|c|}{Attributes:30\% - Geometry:70\%}\\ \hline
    & \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04} & \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}\\ \hline
    pQS & 0.25 & 0.43 & 0.75 & 0.9999 & 0.295 & 0.52 & 0.91 & 0.9999 & 0.262 & 0.4965 & 0.87 & 0.9999 & 0.068 & 0.109 & 0.192 & 0.37 & 0.049 & 0.098 & 0.19 & 0.32 \\ \hline
    QP & 43 & 42 & 40 & 39 & 45 & 44 & 41 & 40 & 40 & 39 & 34 & 33 & 40 & 38 & 36 & 33 & 45 & 44 & 42 & 36 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:40\% - Geometry:60\%}\\ \hline
    pQS & 0.22 & 0.41 & 0.7 & 0.9999 & 0.25 & 0.48 & 0.87 & 0.9999 & 0.252 & 0.4365 & 0.77 & 0.999 & 0.06 & 0.105 & 0.19 & 0.35 & 0.041 & 0.083 & 0.168 & 0.282 \\ \hline
    QP & 40 & 40 & 38 & 36 & 42 & 41 & 38 & 38 & 38 & 36 & 31 & 29 & 37 & 35 & 32 & 29 & 42 & 41 & 39 & 33 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:50\% - Geometry:50\%}\\ \hline
    pQS & 0.185 & 0.36698 & 0.65 & 0.99 & 0.23 & 0.43 & 0.77 & 0.9999 & 0.2165 & 0.3865 & 0.7 & 0.999 & 0.055 & 0.09 & 0.175 & 0.3 & 0.038 & 0.075 & 0.157 & 0.25 \\ \hline
    QP & 37 & 36 & 34 & 32 & 39 & 38 & 36 & 34 & 35 & 33 & 27 & 25 & 34 & 31 & 29 & 26 & 39 & 38 & 36 & 30 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:60\% - Geometry:40\%}\\ \hline
    pQS & 0.75 & 0.31 & 0.6 & 0.99 & 0.19 & 0.36 & 0.69 & 0.89 & 0.19 & 0.3365 & 0.65 & 0.89 & 0.049 & 0.083 & 0.155 & 0.27 & 0.031 & 0.062 & 0.13 & 0.22 \\ \hline
    QP & 34 & 33 & 32 & 30 & 35 & 34 & 32 & 31 & 31 & 30 & 24 & 21 & 30 & 28 & 25 & 21 & 35 & 34 & 32 & 27 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:70\% - Geometry:30\%}\\ \hline
    pQS & 0.155 & 0.285 & 0.5 & 0.88 & 0.17 & 0.29 & 0.58 & 0.79 & 0.166 & 0.28 & 0.55 & 0.88 & 0.04 & 0.069 & 0.135 & 0.23 & 0.026 & 0.05 & 0.11 & 0.2 \\ \hline
    QP & 30 & 31 & 28 & 26 & 31 & 28 & 27 & 26 & 28 & 26 & 21 & 17 & 26 & 23 & 21 & 16 & 30 & 29 & 28 & 25 \\ \hline
    \end{tabular}%
    }\label{tab:parametersPRED}

%\end{table*}
%\begin{table*}[!t]
    \centering
    \caption{Parameters for G-PCC RAHT.}    
    \vspace*{-1.6mm}
   \resizebox{\linewidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Parameter & \multicolumn{4}{|c|}{\textbf{Bouquet}}& \multicolumn{4}{|c|}{\textbf{StMihcael}}& \multicolumn{4}{|c|}{\textbf{Thaidancer}}& \multicolumn{4}{|c|}{\textbf{CITIUSP}} & \multicolumn{4}{|c|}{\textbf{Bumbameuboi}}\\ \hline
    &\multicolumn{20}{|c|}{Attributes:30\% - Geometry:70\%}\\ \hline
    & \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04} & \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}\\ \hline
    pQS & 0.25 & 0.45 & 0.8 & 0.9999 & 0.289 & 0.52 & 0.9 & 0.9999 & 0.26 & 0.509 & 0.85 & 0.9999 & 0.067 & 0.11 & 0.2 & 0.38 & 0.048 & 0.091 & 0.18 & 0.3 \\ \hline
    QP & 40 & 39 & 37 & 36 & 41 & 40 & 37 & 36 & 37 & 36 & 31 & 30 & 36 & 35 & 32 & 30 & 42 & 41 & 39 & 33 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:40\% - Geometry:60\%}\\ \hline
    pQS & 0.239 & 0.42 & 0.7 & 0.9998 & 0.256 & 0.504 & 0.86 & 0.9999 & 0.25 & 0.43 & 0.77 & 0.999 & 0.063 & 0.1 & 0.18 & 0.34 & 0.043 & 0.081 & 0.17 & 0.27 \\ \hline
    QP & 38 & 37 & 34 & 33 & 38 & 38 & 35 & 34 & 35 & 33 & 28 & 27 & 34 & 32 & 30 & 27 & 40 & 38 & 36 & 31 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:50\% - Geometry:50\%}\\ \hline
    pQS & 0.21 & 0.37 & 0.65 & 0.999 & 0.246 & 0.44 & 0.76 & 0.999 & 0.21 & 0.4 & 0.7 & 0.999 & 0.058 & 0.092 & 0.165 & 0.31 & 0.038 & 0.071 & 0.15 & 0.25 \\ \hline
    QP & 35 & 34 & 32 & 29 & 36 & 35 & 32 & 31 & 32 & 31 & 25 & 22 & 31 & 29 & 27 & 22 & 36 & 35 & 33 & 28 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:60\% - Geometry:40\%}\\ \hline
    pQS & 0.17 & 0.32 & 0.6 & 0.99 & 0.2 & 0.36 & 0.7 & 0.999 & 0.18 & 0.34 & 0.66 & 0.999 & 0.049 & 0.081 & 0.14 & 0.27 & 0.032 & 0.061 & 0.125 & 0.22 \\ \hline
    QP & 32 & 31 & 30 & 27 & 32 & 31 & 29 & 27 & 29 & 28 & 22 & 18 & 27 & 26 & 22 & 19 & 33 & 32 & 30 & 26 \\ \hline
    &\multicolumn{20}{|c|}{Attributes:70\% - Geometry:30\%}\\ \hline
    pQS & 0.15 & 0.275 & 0.53 & 0.89 & 0.18 & 0.33 & 0.6 & 0.88 & 0.15 & 0.28 & 0.53 & 0.89 & 0.041 & 0.073 & 0.132 & 0.235 & 0.027 & 0.05 & 0.107 & 0.2 \\ \hline
    QP & 28 & 28 & 27 & 24 & 29 & 28 & 26 & 20 & 26 & 24 & 19 & 14 & 24 & 22 & 19 & 14 & 29 & 28 & 27 & 24 \\ \hline
    \end{tabular}%
    }\label{tab:parametersRAHT}
\end{table*}
%\begin{table*}
%    \centering
%    \caption{Parameters for JPEG VM.}
%   \resizebox{\linewidth}{!}{%
%    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%    \hline
%    Parameter & \multicolumn{4}{|c|}{\textbf{Bouquet}}& \multicolumn{4}{|c|}{\textbf{StMihcael}}& \multicolumn{4}{|c|}{\textbf{Thaidancer}}& \multicolumn{4}{|c|}{\textbf{CITIUSP}} & \multicolumn{4}{|c|}{\textbf{Bumbameuboi}}\\ \hline
%    &\multicolumn{20}{|c|}{Attributes:30\% - Geometry:70\%}\\ \hline
%    & \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04} & \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}& \textbf{R01} & \textbf{R02} & \textbf{R03} & \textbf{R04}\\ \hline
%    Lambda & 0.0025 & 0.0025 & 0.01 & 0.0025 & 0.025 & 0.01 & 0.01 & 0.003 & 0.05 & 0.0025 & 0.0025 & 0.005 & 0.025 & 0.01 & 0.01 & 0.005 & 0.025 & 0.003 & 0.01 & 0.005 \\ \hline
%    BS & 32 & 64 & 128 & 128 & 32 & 64 & 128 & 128 & 32 & 32 & 64 & 128 & 32 & 64 & 128 & 128 & 32 & 32 & 128 & 128 \\ \hline
%    SF & 4 & 2 & 1 & 1 & 4 & 2 & 1 & 1 & 4 & 4 & 2 & 1 & 4 & 2 & 1 & 1 & 4 & 4 & 1 & 1 \\ \hline
%    SR & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 1 & 0 & 0 \\ \hline
%    ColIDX & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 2 & 2 & 1 & 0 & 0 & 0 & 1 & 0 & 2 & 0 & 1 \\ \hline
%    &\multicolumn{20}{|c|}{Attributes:40\% - Geometry:60\%}\\ \hline
%    Lambda & 0.025 & 0.005 & 0.0025 & 0.0025 & 0.005 & 0.005 & 0.005 & 0.0025 & 0.025 & 0.01 & 0.01 & 0.0025 & 0.05 & 0.025 & 0.0025 & 0.005 & 0.025 & 0.0025 & 0.005 & 0.0025 \\ \hline
%    BS & 64 & 64 & 64 & 128 & 32 & 64 & 128 & 128 & 32 & 64 & 128 & 128 & 32 & 128 & 64 & 128 & 32 & 32 & 64 & 64 \\ \hline
%    SF & 2 & 2 & 2 & 1 & 4 & 2 & 1 & 1 & 4 & 2 & 1 & 1 & 4 & 1 & 2 & 1 & 4 & 4 & 2 & 2 \\ \hline
%    SR & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 1 & 1 & 0 \\ \hline
%    ColIDX & 0 & 1 & 2 & 2 & 1 & 1 & 1 & 2 & 1 & 1 & 1 & 3 & 0 & 0 & 3 & 2 & 1 & 3 & 2 & 3 \\ \hline
%    &\multicolumn{20}{|c|}{Attributes:50\% - Geometry:50\%}\\ \hline
%    Lambda & 0.005 & 0.01 & 0.005 & 0.005 & 0.05 & 0.01 & 0.005 & 0.0025 & 0.05 & 0.01 & 0.005 & 0.0025 & 0.025 & 0.01 & 0.01 & 0.005 & 0.05 & 0.01 & 0.005 & 0.0025 \\ \hline
%    BS & 32 & 64 & 64 & 64 & 64 & 64 & 128 & 128 & 64 & 64 & 128 & 128 & 32 & 64 & 128 & 128 & 32 & 64 & 64 & 64 \\ \hline
%    SF & 4 & 2 & 2 & 1 & 2 & 2 & 1 & 1 & 2 & 2 & 1 & 1 & 4 & 2 & 1 & 1 & 4 & 2 & 2 & 2 \\ \hline
%    SR & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 1 & 1 \\ \hline
%    ColIDX & 2 & 1 & 2 & 2 & 0 & 1 & 2 & 3 & 0 & 1 & 2 & 3 & 1 & 1 & 1 & 3 & 1 & 2 & 3 & 4 \\ \hline
%   &\multicolumn{20}{|c|}{Attributes:60\% - Geometry:40\%}\\ \hline
%    Lambda & 0.01 & 0.025 & 0.01 & 0.0025 & 0.05 & 0.01 & 0.01 & 0.005 & 0.05 & 0.005 & 0.005 & 0.005 & 0.01 & 0.0025 & 0.01 & 0.0025 & 0.05 & 0.005 & 0.01 & 0.01 \\ \hline
%    BS & 32 & 64 & 64 & 128 & 32 & 64 & 128 & 128 & 32 & 32 & 64 & 128 & 32 & 32 & 128 & 128 & 32 & 32 & 64 & 64 \\ \hline
%    SF & 4 & 2 & 2 & 1 & 4 & 2 & 1 & 1 & 4 & 4 & 2 & 1 & 4 & 4 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
%    SR & 1 & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 1 & 1 \\ \hline
%    ColIDX & 2 & 1 & 2 & 3 & 1 & 2 & 2 & 4 & 2 & 4 & 4 & 4 & 2 & 3 & 2 & 3 & 2 & 4 & 3 & 3 \\ \hline
%    &\multicolumn{20}{|c|}{Attributes:70\% - Geometry:30\%}\\ \hline
%    Lambda & 0.025 & 0.025 & 0.05 & 0.01 & 0.05 & 0.025 & 0.0025 & 0.01 & 0.05 & 0.01 & 0.05 & 0.01 & 0.05 & 0.025 & 0.005 & 0.01 & 0.05 & 0.01 & 0.01 & 0.01 \\ \hline
%    BS & 32 & 64 & 64 & 128 & 32 & 64 & 64 & 128 & 32 & 32 & 128 & 128 & 32 & 64 & 64 & 128 & 64 & 32 & 64 & 128 \\ \hline
%    SF & 4 & 2 & 1 & 1 & 4 & 2 & 2 & 1 & 4 & 4 & 1 & 1 & 4 & 2 & 2 & 1 & 2 & 4 & 2 & 1 \\ \hline
%    SR & 1 & 1 & 0 & 0 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 1 & 0 & 0 \\ \hline
%    ColIDX & 2 & 2 & 1 & 3 & 2 & 2 & 4 & 3 & 3 & 4 & 2 & 4 & 2 & 2 & 4 & 3 & 1 & 4 & 3 & 3 \\ \hline
%    \end{tabular}%
%    }\label{tab:parametersJPEGVM}
\%end{table*}
